Self-force corrections to the periapsis advance around a spinning black hole

The linear in mass ratio correction to the periapsis advance of equatorial orbits around a spinning black hole is calculated for the first time and to very high precision, providing a key benchmark for different approaches modelling spinning binaries. The high precision of the calculation is leveraged to discriminate between two recent incompatible derivations of the 4PN equations of motion. Finally, the limit of the periapsis advance near the innermost stable orbit (ISCO) allows determination of the ISCO shift, validating previous calculations using the first law of binary mechanics. Calculation of the ISCO shift is further extended into the near extremal regime (with spins up to $1-a=10^{-20}$), revealing new unexpected phenomenology. In particular, we find that the shift of the ISCO does not have a well defined extremal limit, but instead continues to oscillate.

==> commands.tex <==
\newtheorem{lem}{Lemma}
\newcommand{\TabH}[1]{\multicolumn{1}{c}{#1}}

\newcommand{\RR}{\mathbbm{R}}					%Real numbers
\newcommand{\CC}{\mathbbm{C}}					%Complex numbers
\newcommand{\NN}{\mathbbm{N}}					%Natural numbers
\newcommand{\ZZ}{\mathbbm{Z}}					%Integers

\newcommand{\abs}[1]{\lvert#1\rvert}			%Absolute value
\newcommand{\norm}[1]{\lVert#1\rVert}			%Norm
\newcommand{\avg}[1]{\left\langle #1 \right\rangle }		%Average

\newcommand{\cb}[1]{\left\{#1\right\} }			%Scaling curly braces
\newcommand{\cbb}[1]{\big\{#1\big\} }			%big curly braces
\newcommand{\cbB}[1]{\Big\{#1\Big\} }			%Big curly braces
\newcommand{\hh}[1]{\left(#1\right) }			%Scaling parentheses
\newcommand{\nh}[1]{(#1) }						%normal parentheses
\newcommand{\bh}[1]{\bigl(#1\bigr) }			%big parentheses
\newcommand{\Bh}[1]{\Bigr(#1\Bigr) }			%Big parentheses
\newcommand{\bbh}[1]{\biggl(#1\biggr) }			%bigg parentheses
\newcommand{\BBh}[1]{\Biggr(#1\Biggr) }			%Bigg parentheses

\newcommand{\U}{\Upsilon}						%Mino frequency
\newcommand{\q}{q}								%Mino phase
\newcommand{\e}{\epsilon}						%Mass ratio

\newcommand{\id}[1]{\operatorname{d}\!#1}												%Differential
\renewcommand{\d}[2]{\frac{\operatorname{d}\!#1}{\operatorname{d}\!#2}}					%Derivative
\newcommand{\dd}[2]{\frac{\operatorname{d}^2\!#1}{\operatorname{d}\!#2^2}}				%Double derivative
\newcommand{\pd}[2]{\frac{\operatorname{\partial}\!#1}{\operatorname{\partial}\!#2}}	%Partial derivative
\newcommand{\CD}[1]{\nabla_{#1}}

\newcommand{\ii}{i}								%Imaginary unit
\newcommand{\ee}{e}								%Natural base

\newcommand{\pt}{\tau}							%proper time
\newcommand{\mt}{\lambda}						%Mino time
\newcommand{\COM}{K}

\newcommand{\nE}{\mathcal{E}}								%Specific energy
\newcommand{\nL}{\mathcal{L}}							%Specific angular momentum
\newcommand{\nQ}{Q}								%Specific Carter constant
\newcommand{\nEd}{\dot{\nE}}
\newcommand{\nLd}{\dot{L}_z}
\newcommand{\nQd}{\dot{\nQ}}

\newcommand{\rmin}{r_\mathrm{min}}
\newcommand{\rmax}{r_\mathrm{max}}
\newcommand{\zmax}{z_\mathrm{max}}

\newcommand{\mr}{\eta}

\newcommand{\ptrp}{\mathcal{T}_r}
\newcommand{\ctrp}{T_r}
\newcommand{\mtrp}{\Lambda_r}

\DeclareMathOperator{\bigO}{\mathcal{O}}					%Big O notation
\DeclareMathOperator{\sign}{sign}				%Sign

\newcommand{\tet}[2]{e_{#1}^{#2}}				%tetrad
\newcommand{\itet}[2]{e^{#1}_{#2}}				%inverse tetrad

\newcommand{\R}[3][]{\,{_{#2}R_{#3}^{\mathrm{#1}}}}		%Homogeneous solution of the radial teukolsky eq.
\newcommand{\Rb}[3][]{\,{_{#2}\bar{R}_{#3}^{\mathrm{#1}}}}		%Homogeneous solution of the radial teukolsky eq.
\newcommand{\SWSH}[3][]{\,{_{#2}S_{#3}^{\mathrm{#1}}}}	%Spin-weighted spheroidal harmonic
\newcommand{\Y}[3][]{\,{_{#2}Y_{#3}^{\mathrm{#1}}}}		%Spin-weighted spherical harmonic
\newcommand{\T}[3][]{\,{_{#2}T_{#3}^{\mathrm{#1}}}}		%Teukolsky source

\newcommand{\Sb}[4]{({_{#1}b_{#2}})^{#3}_{#4}}			%spheroidal-to-spherical projector
\newcommand{\YA}[4]{\tensor*[_{#1\hspace{3pt}}^{#2}]{\hspace{-3pt}\mathcal{A}}{^{#3}_{#4}}
%{_{#1}^{\hfill#2}\hspace{-1.25pt}\mathcal{A}^{#3}_{#4}}
}			%spheroidal-to-spherical projector
\newcommand{\YB}[4]{{^{#1#2}\!\mathcal{B}^{#3}_{#4}}}			%spheroidal-to-spherical projector

\newcommand{\TEV}[2]{\,{_{#1}\lambdabar_{#2}}}			%Radial teukolsky EV
\newcommand{\SEV}[2]{\,{_{#1}A_{#2}}}					%SWSH eigenvalue

\newcommand{\A}[3][]{{_{#2}A_{#3}^{\mathrm{#1}}}}		%Down going coefficient at horizon
\newcommand{\B}[3][]{{_{#2}B_{#3}^{\mathrm{#1}}}}		%Up going coefficient at horizon

\newcommand{\Ainf}[3][]{{_{#2}\alpha_{#3}^{\mathrm{#1}}}}	%incoming coefficient at infinity
\newcommand{\Binf}[3][]{{_{#2}\beta_{#3}^{\mathrm{#1}}}}	%outgoing coefficient at infinity

\newcommand{\Ab}[3][]{{_{#2}\bar{A}_{#3}^{\mathrm{#1}}}}		%Down going coefficient at horizon
\newcommand{\Bb}[3][]{{_{#2}\bar{B}_{#3}^{\mathrm{#1}}}}		%Up going coefficient at horizon

\newcommand{\Ainfb}[3][]{{_{#2}\bar{\alpha}_{#3}^{\mathrm{#1}}}}	%incoming coefficient at infinity
\newcommand{\Binfb}[3][]{{_{#2}\bar{\beta}_{#3}^{\mathrm{#1}}}}	%outgoing coefficient at infinity


\newcommand{\ph}[2]{(#1)_{#2}}			%Pochhammer


\newcommand{\pI}{+}						%Physical at infinity
\newcommand{\uI}{\not{+}}				%Unphysical at infinity
\newcommand{\pH}{-}						%Physical at horizon
\newcommand{\uH}{\not{-}}				%Unphysical at Horizon
\newcommand{\pIH}{\pm}					%Physical at Infinity/Horizon
\newcommand{\uIH}{\not{\pm}}			%Unphysical at Infinity/Horizon
\newcommand{\pHI}{\mp}					%Physical atHorizon/ Infinity
\newcommand{\uHI}{\not{\mp}}			%Unphysical at Horizon/Infinity



\newcommand{\F}{{_{2}F_1}}				%Hypergeometric Function
\newcommand{\lP}[3]{P_{#1}^{#2}(#3)}	%Legendre P
\newcommand{\lQ}[3]{Q_{#1}^{#2}(#3)}	%legendre Q

\newcommand{\MROP}[1]{\hat{\mathcal{H}}_{#1}}	%Metric reconstruction operator


\newcommand{\MC}{\mathcal{C}}					%Magic constant

\newcommand{\SWL}[1]{\bar\eth_{#1}}				%Ethbar
\newcommand{\TP}{\epsilon}						%Target precision

\newcommand{\spl}{\mathfrak{l}}					%spheroidal l-mode

\newcommand{\lmax}{l_\mathrm{max}}				%l_max
\newcommand{\llmax}{\spl_{\mathrm{max}}}		%spheroidal l_max
\newcommand{\kmax}{k_\mathrm{max}}				%k_max
\newcommand{\Lmax}{L_\mathrm{max}}				%L_max
\newcommand{\Lmin}{L_\mathrm{min}}				%L_min

\newcommand{\ret}{\mathrm{Ret}}
\newcommand{\adv}{\mathrm{Adv}}
\newcommand{\reg}{\mathrm{R}}
\newcommand{\sing}{\mathrm{S}}

\newcommand{\diss}{\mathrm{diss}}
\newcommand{\cons}{\mathrm{cons}}

\newcommand{\Lor}{\mathrm{Lor}}
\newcommand{\Rad}{\mathrm{Rad}}
\newcommand{\Avg}{\mathrm{Avg}}

\newcommand{\RP}[1]{\mathcal{E}_{#1}}

\newcommand{\pISO}{p_\mathrm{ISO}}

\newcommand{\mvdm}[1]{{\color{red} (MvdM: #1)}}

\DeclareMathOperator{\Dop}{\hat{D}}
\DeclareMathOperator{\Delop}{\hat{\Delta}}
\DeclareMathOperator{\delop}{\hat{\delta}}
\DeclareMathOperator{\delopbar}{\hat{\bar{\delta}}}

\newcommand{\Fext}{\mathcal{F}} 						% Self-force extension

%\DeclareMathOperator{\umin}{\scalebox{1}[1]{-}}
\newcommand{\umin}{\mathord{\scalebox{0.75}[1]{\(-\)}}}

\newcommand\Ts{\rule{0pt}{2.6ex}}       % Top strut for vertical spacing in tables
\newcommand\Bs{\rule[-1.2ex]{0pt}{0pt}} % Bottom strut

\newcommand{\solarmass}{M_{\astrosun}}
